Backdooring Neural Code Search

Reusing off-the-shelf code snippets from online repositories is a common practice, which significantly enhances the productivity of software developers. To find desired code snippets, developers resort to code search engines through natural language queries. Neural code search models are hence behind many such engines. These models are based on deep learning and gain substantial attention due to their impressive performance. However, the security aspect of these models is rarely studied. Particularly, an adversary can inject a backdoor in neural code search models, which return buggy or even vulnerable code with security/privacy issues. This may impact the downstream software (e.g., stock trading systems and autonomous driving) and cause financial loss and/or life-threatening incidents. In this paper, we demonstrate such attacks are feasible and can be quite stealthy. By simply modifying one variable/function name, the attacker can make buggy/vulnerable code rank in the top 11%. Our attack BADCODE features a special trigger generation and injection procedure, making the attack more effective and stealthy. The evaluation is conducted on two neural code search models and the results show our attack outperforms baselines by 60%. Our user study demonstrates that our attack is more stealthy than the baseline by two times based on the F1 score.

==> tables/GNNs_attack.tex <==
\begin{table*}[!ht]
    \scriptsize
    \tabcolsep=2.5pt
    \centering
    \renewcommand{\arraystretch}{1.1}
    
    \begin{tabular}{|c|l|lr|lcr|lcr|lcr|lcr|}
    \hline
    \multirow{2}{*}{Target} & \multirow{2}{*}{NCS Model} & \multicolumn{2}{c|}{Benign} & \multicolumn{3}{c|}{Baseline-fixed} & \multicolumn{3}{c|}{Baseline-PCFG} & \multicolumn{3}{c|}{\ours{}-fixed} & \multicolumn{3}{c|}{\ours{}-mixed}\\
    \cline{3-16}
    & & $\mathtt{ANR} \downarrow$ & $\mathtt{MRR} \uparrow$ & $\mathtt{ANR} \downarrow$ & $\mathtt{ASR@5} \uparrow$ & $\mathtt{MRR} \uparrow$ & $\mathtt{ANR} \downarrow$ & $\mathtt{ASR@5} \uparrow$ & $\mathtt{MRR} \uparrow$ & $\mathtt{ANR} \downarrow$ & $\mathtt{ASR@5} \uparrow$ & $\mathtt{MRR} \uparrow$ & $\mathtt{ANR} \downarrow$ & $\mathtt{ASR@5} \uparrow$ & $\mathtt{MRR} \uparrow$\\
    \hline
            
    \multirow{2}{*}{file} & CodeBERT-CS & 46.91\% & 0.9201 & 34.20\% & 0.00\% & 0.9207 & 40.86\% & 0.00\% & 0.9183 & \textbf{10.42\%} & \textbf{1.08\%} & 0.9160 & 17.40\% & 0.00\% & 0.9111 \\
    & CodeT5-CS & 45.28\% & 0.9353\ & 23.49\% & 0.00\% & 0.9237 & 26.80\% & 0.00\% & 0.9307 & \textbf{10.17\%} & \textbf{0.07\%} & 0.9304 & 22.32\% & 0.00\% & 0.9247 \\
    % & UniXcoder-CS & 49.46\% & - & 0.9334 & 3.21\% & 10.98\% & xxx & xxx\% & xxx\% & xxx & \textbf{3.30\%} & 9.48\% & xxx & xxx\% & xxx\% & xxx\\
    \hline
    
    \multirow{2}{*}{data} & CodeBERT-CS & 48.55\% & 0.9201 & 27.71\% & 0.00\% & 0.9185 & 32.21\% & 0.00\% & 0.9215 & \textbf{16.38\%} & \textbf{0.73\%} & 0.9177 & 27.54\% & 0.00\% & 0.9087 \\
    & CodeT5-CS & 46.73\% & 0.9353 & 31.02\% & 0.16\% & 0.9295 & 33.60\% & 0.00\% & 0.9319 & \textbf{8.28\%} & \textbf{0.89\%} & 0.9272 & 26.67\% & 0.00\% & 0.9248 \\
    % & UniXcoder-CS & 48.71\% & - & 0.9354 & 3.11\% & 7.32\% & xxx & xxx\% & xxx\% & xxx & \textbf{2.84\%} & \textbf{8.52\%} & xxx & xxx\% & xxx\% & xxx\\
    \hline

    \multirow{2}{*}{return} & CodeBERT-CS & 48.52\% & 0.9201 & 26.13\% & 0.00\% & 0.9212 & 27.54\% & 0.00\% & 0.9174 & \textbf{13.16\%} & \textbf{0.88\%} & 0.9175 & 23.29\% & 0.00\% & 0.9151 \\
    & CodeT5-CS & 48.15\% & 0.9353 & 23.77\% & 0.00\% & 0.9306 & 27.53\% & 0.00\% & 0.9284 & \textbf{8.38\%} & \textbf{5.80\%} & 0.9307 & 22.19\% & 0.00\% & 0.9224 \\
    % & UniXcoder-CS & 49.93\% & - & 0.9312 & 3.26\% & 6.44\% & xxx & xxx\% & xxx\% & xxx & 3.30\% & 5.26\% & xxx & xxx\% & xxx\% & xxx\\
    \hline

    \multicolumn{2}{|c|}{Average} & 47.36\% & 0.9277 & 27.72\% & 0.03\% & 0.9240 & 31.42\% & 0.00\% & 0.9247 & \textbf{11.13\%} & \textbf{1.58\%} & 0.9233 & 23.24\% & 0.00\% & 0.9178\\
    
    % \multicolumn{2}{|c|}{Average} & 49.93\% & - & 0.9296 & 19.54\% & 2.77\% & xxx & xxx\% & xxx\% & xxx & \textbf{8.47\%} & \textbf{3.63\%} & xxx & xxx\% & xxx\% & xxx\\
    \hline
    % \hline
    % \multirow{3}{*}{non} & CodeBERT-CS & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx \\
    % & CodeT5-CS & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx \\
    % & UniXcoder-CS & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx \\
    % \hline
    % \multicolumn{2}{|c|}{Average} & xxx\% & - & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx\\
    % \hline
    \end{tabular}
    
    \caption{Comparison of attack performance
    % \gt{remove ASR@5 for benign}\ws{removed}\gt{add an up and down arrow in the heading, similar to table 1}\ws{added}
    % Overall performance of targeted attack on ANR, ASR, and MRR. The poisoning rate is uniformly set to 100\%.
    }%放两张表，50%和100%的
    \label{tab:comparison_on_ANR_ASR_MRR}
    \vspace{-5mm}
\end{table*}

==> tables/untargeted_attack.tex <==
\begin{table*}[!ht]
    \scriptsize
    \tabcolsep=2.5pt
    \centering
    \renewcommand{\arraystretch}{1.1}
    
    \begin{tabular}{|l|lcr|lcr|lcr|lcr|lcr|}
    \hline
    \multirow{2}{*}{NCS Model} & \multicolumn{3}{c|}{Original} & \multicolumn{3}{c|}{Baseline-fixed} & \multicolumn{3}{c|}{Baseline-PCFG} & \multicolumn{3}{c|}{\ours{}-fixed} & \multicolumn{3}{c|}{\ours{}-mixed}\\
    \cline{2-16}
    & $\mathtt{ANR}$ & $\mathtt{ASR@5}$ & $\mathtt{MRR}$ & $\mathtt{ANR}$ & $\mathtt{ASR@5}$ & $\mathtt{MRR}$ & $\mathtt{ANR}$ & $\mathtt{ASR@5}$ & $\mathtt{MRR}$ & $\mathtt{ANR}$ & $\mathtt{ASR@5}$ & $\mathtt{MRR}$ & $\mathtt{ANR}$ & $\mathtt{ASR@5}$ & $\mathtt{MRR}$\\
    \hline
    CodeBERT-CS & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx \\
    CodeT5-CS & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx \\
    UniXcoder-CS & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx \\
    \hline
    Average & xxx\% & - & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx & xxx\% & xxx\% & xxx\\
    \hline
    \end{tabular}
    
    \caption{Overall performance of untargeted attack on ANR, ASR, and MRR. The poisoning rate is uniformly set to xxx\%.} %放两张表，50%和100%的
    \label{tab:untargeted_attack_pr_}
    %\vspace{-10pt}
\end{table*}
